Semantic Noise Reduction via Teacher-Guided Dual-Path Audio-Visual Representation Learning

Recent advances in audio-visual representation learning have shown the value of combining contrastive alignment with masked reconstruction. However, jointly optimizing these objectives in a single forward pass forces the contrastive branch to rely on randomly visible patches designed for reconstruction rather than cross-modal alignment, introducing semantic noise and optimization interference. We propose TG-DP, a Teacher-Guided Dual-Path framework that decouples reconstruction and alignment into separate optimization paths. By disentangling the masking regimes of the two branches, TG-DP enables the contrastive pathway to use a visibility pattern better suited to cross-modal alignment. A teacher model further provides auxiliary guidance for organizing visible tokens in this branch, helping reduce interference and stabilize cross-modal representation learning. TG-DP achieves state-of-the-art performance in zero-shot retrieval. On AudioSet, it improves R@1 from 35.2\% to 37.4\% for video-to-audio retrieval and from 27.9\% to 37.1\% for audio-to-video retrieval. The learned representations also remain semantically robust, achieving state-of-the-art linear-probe performance on AS20K and VGGSound. Taken together, our results suggest that decoupling multimodal objectives and introducing teacher-guided structure into the contrastive pathway provide an effective framework for improving large-scale audio-visual pretraining. Code is available at https://github.com/wanglg20/TG-DP.

==> tables/denseAV.tex <==
\vspace{-4pt}
\begin{table}[!ht]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l ccc ccc}
\toprule
\textbf{Method}
& \multicolumn{3}{c}{\textbf{VGGSound V$\rightarrow$A}}
& \multicolumn{3}{c}{\textbf{VGGSound A$\rightarrow$V}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
& R@1 & R@5 & R@10 & R@1 & R@5 & R@10 \\
\midrule
DenseAV & 24.2 & 48.2 & 58.3 & 25.1 & 50.1 & 59.1 \\
Ours (TG-DP) & \textbf{31.3} & \textbf{54.4} & \textbf{63.9}
             & \textbf{30.3} & \textbf{53.1} & \textbf{64.3} \\
\bottomrule
\end{tabular}
\caption{Comparison with DenseAV on VGGSound retrieval.}
\label{tab:rebuttal_denseav}
\end{table}


==> tables/ex_detail.tex <==
\noindent
\begin{minipage}{1\linewidth}
\small
\raggedright
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{lccc}
\toprule
\textbf{Setting} & \textbf{Pretrain} & \textbf{AS20K LP} & \textbf{VGG LP} \\
\midrule
Dataset & AS-2M & AS-20K & VGGSound \\
Optimizer & Adam & Adam & Adam \\
Learning Rate & $2\!\times\!10^{-4}$ & $5\!\times\!10^{-2}$ & $1\!\times\!10^{-3}$ \\
LR Scheduler & Cosine & Cosine & Cosine \\
Epochs & \textbf{35} & 15 & 10 \\
Warmup Epochs & \textbf{3.5} & 1.5 & 1 \\
Batch Size & $8\times 64$ & 48 & 48 \\
GPUs & \textbf{8$\times$H100} & 2$\times$H100 & 2$\times$H100 \\
Audio Input Size & 128$\times$416 & $16\times$128$\times$416 & $16\times$128$\times$416 \\
Class-Balanced & No & No & Yes \\
Mixup & No & Yes & Yes \\
Random Shift & Yes & Yes & Yes \\
Loss Function & --- & BCE & CE \\
Weight Averaging & No & Yes & Yes \\
Norm Mean & $-5.081$ & $-5.081$ & $-5.081$ \\
Norm STD & 4.485 & 4.485 & 4.485 \\
\bottomrule
\end{tabular}
\captionof{table}{Hyperparameters for pretraining and linear probing.}
\label{tab:pretrain-lp}
\end{minipage}


==> tables/rebuttal.tex <==


\begin{table}[!ht]
\centering
\setlength{\tabcolsep}{6.5pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{l ccc ccc c}
\toprule
\textbf{Mask Ratio} 
& \multicolumn{3}{c}{\textbf{VGGSound (V$\rightarrow$A)}} 
& \multicolumn{3}{c}{\textbf{VGGSound (A$\rightarrow$V)}} 
& \textbf{Classification} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-8}
& R@1 & R@5 & R@10 & R@1 & R@5 & R@10 & AS20K (mAP) \\
\midrule
0.00 & 30.4{(-0.9)} & 56.0{(+1.6)} & 64.2{(+0.3)} & 29.8{(-0.5)} & 55.6{(+2.5)} & 64.5{(+0.2)} & 29.6{(-2.4)}\\
0.50 & 31.3 & 54.4 & 63.9 & 30.3 & 53.1 & 64.3 & \textbf{32.0} \\
\bottomrule
\end{tabular}
}
\caption{Ablation on contrastive-branch mask ratio (0.00 vs. 0.50).}
\label{tab:ablation_maskratio}
\end{table}
\vspace{-6pt}   % 表格后
